Uniform Priors for Data-Efficient Transfer

Deep Neural Networks have shown great promise on a variety of downstream applications; but their ability to adapt and generalize to new data and tasks remains a challenge. However, the ability to perform few or zero-shot adaptation to novel tasks is important for the scalability and deployment of machine learning models. It is therefore crucial to understand what makes for good, transfer-able features in deep networks that best allow for such adaptation. In this paper, we shed light on this by showing that features that are most transferable have high uniformity in the embedding space and propose a uniformity regularization scheme that encourages better transfer and feature reuse. We evaluate the regularization on its ability to facilitate adaptation to unseen tasks and data, for which we conduct a thorough experimental study covering four relevant, and distinct domains: few-shot Meta-Learning, Deep Metric Learning, Zero-Shot Domain Adaptation, as well as Out-of-Distribution classification. Across all experiments, we show that uniformity regularization consistently offers benefits over baseline methods and is able to achieve state-of-the-art performance in Deep Metric Learning and Meta-Learning.

==> tables/dml_table.tex <==
\begin{table*}[t!]
 \small
 \begin{minipage}[c]{\textwidth}
   \setlength\tabcolsep{1.4pt}
   \centering
%   \resizebox{\textwidth}{!}{
    \caption{\textbf{Deep Metric Learning (Zero-Shot Generalization)}. Comparison of several deep metric learning objectives with a ResNet-50 backbone \citep{resnet} on two standard benchmarks: CUB200-2011 \citep{birds} \& CARS196 \citep{cars}.
    The models are evaluated with and without max-entropy regularization and
    we report the mean Recall@1 and the Normalized Mutual Information (NMI) metric for all experiments.
    All baseline scores are taken from \cite{roth2020revisiting}, and 
    their 
    \href{https://github.com/Confusezius/Revisiting_Deep_Metric_Learning_PyTorch}{official released code}
    is used to run all experiments without any fine-tuning for the underlying 
    metric learning model hyperparameters.}
    
   \begin{tabular}{l || c | c || c | c}
     \toprule
     \multicolumn{1}{l}{\textbf{Benchmarks}$\rightarrow$} & \multicolumn{2}{c}{CUB200-2011} & \multicolumn{2}{c}{CARS196} \\
%      & \multicolumn{2}{|c|}{\citep{birds}} & \multicolumn{2}{c}{\citep{cars}} \\
     \midrule
     \textbf{Method}$\downarrow$ & R@1 & NMI & R@1 & NMI \\
     \midrule
    Softmax \citep{softmax} & 61.7 $\pm$ 0.3 & 66.8 $\pm$ 0.4 & 78.9 $\pm$ 0.3 & 66.4 $\pm$ 0.3 \\
    \rowcolor[HTML]{EFEFEF}
    Softmax + Entropy &  \textbf{65.0} $\pm$ 0.1 & \textbf{68.8} $\pm$ 0.2 & \textbf{80.6} $\pm$ 0.2 & \textbf{68.3} $\pm$ 0.2 \\
%    Quadruplet \citep{qaudrupletloss} & 61.71 $\pm$ 0.63 & 66.60 $\pm$ 0.41 & 76.34 $\pm$ 0.27 & 64.79 $\pm$ 0.50 \\
%    Quadruplet + Entropy & \textbf{62.96} $\pm$ 0.58 & \textbf{67.71} $\pm$ 0.25 &  &  \\
    % \midrule 
    % Contrastive \citep{contrastive} & 61.5 $\pm$ 0.2 & 66.5 $\pm$ 0.3 & 75.8 $\pm$ 0.4 & 64.0 $\pm$ 0.2 \\
    % \rowcolor[HTML]{EFEFEF}
    % Contrastive + Entropy & \textbf{63.3} $\pm$ 0.2 & \textbf{67.5} $\pm$ 0.3 & \textbf{76.9} $\pm$ 0.4 & \textbf{65.1} $\pm$ 0.2 \\
    \midrule
    Margin (D, $1.2$) \citep{wu2017sampling} & 63.1 $\pm$ 0.5 & 68.2 $\pm$ 0.3 & 79.9 $\pm$ 0.3 & 67.4 $\pm$ 0.3 \\
    \rowcolor[HTML]{EFEFEF}
    Margin (D, $1.2$) + Entropy & \textbf{65.0} $\pm$ 0.3 & \textbf{69.5} $\pm$ 0.2 & \textbf{82.5} $\pm$ 0.1 & \textbf{68.9} $\pm$ 0.2 \\
    \midrule
    Multisimilarity \citep{multisimilarity} & 62.8 $\pm$ 0.7 & 68.6 $\pm$ 0.4 & 81.7 $\pm$ 0.2 & 69.4 $\pm$ 0.4 \\
    \rowcolor[HTML]{EFEFEF}
    Multisimilarity + Entropy & \textbf{65.4} $\pm$ 0.4 & \textbf{70.3} $\pm$ 0.3 & \textbf{82.2} $\pm$ 0.2 & \textbf{70.5} $\pm$ 0.3 \\
    \bottomrule
    \end{tabular}
    \label{tab:DML_resutls}
    \end{minipage}
 \end{table*}



% \begin{table*}[t!]
%  \small
%  \begin{minipage}[c]{\textwidth}
%   \setlength\tabcolsep{1.4pt}
%   \centering
% %   \resizebox{\textwidth}{!}{
%     \caption{\textbf{Deep Metric Learning (Zero-Shot Generalization)}. Comparison of several deep metric learning objectives with a ResNet-50 backbone \citep{resnet} on two standard benchmarks: CUB200-2011 \citep{birds} \& CARS196 \citep{cars}.
%     The models are evaluated with and without max-entropy regularization and
%     we report the mean Recall \@ 1 and the Normalized Mutual Information (NMI) metric for all experiments.
%     All baseline scores are taken from \cite{roth2020revisiting}, and 
%     their 
%     \href{https://github.com/Confusezius/Revisiting_Deep_Metric_Learning_PyTorch}{official released code}
%     is used to run all experiments without any fine-tuning for the underlying 
%     metric learning model hyperparameters.}
    
%   \begin{tabular}{l || c | c || c | c}
%      \toprule
%      \multicolumn{1}{l}{\textbf{Benchmarks}$\rightarrow$} & \multicolumn{2}{c}{CUB200-2011} & \multicolumn{2}{c}{CARS196} \\
% %      & \multicolumn{2}{|c|}{\citep{birds}} & \multicolumn{2}{c}{\citep{cars}} \\
%      \midrule
%      \textbf{Method}$\downarrow$ & R@1 & NMI & R@1 & NMI \\
%      \midrule
%     Softmax \citep{softmax} & 61.66 $\pm$ 0.30 & 66.77 $\pm$ 0.36 & 78.91 $\pm$ 0.27 & 66.35 $\pm$ 0.30 \\
%     \rowcolor[HTML]{EFEFEF}
%     Softmax + Entropy &  \textbf{65.02} $\pm$ 0.13 & \textbf{68.76} $\pm$ 0.16 & \textbf{80.58} $\pm$ 0.21 & \textbf{68.30} $\pm$ 0.21 \\
% %    Quadruplet \citep{qaudrupletloss} & 61.71 $\pm$ 0.63 & 66.60 $\pm$ 0.41 & 76.34 $\pm$ 0.27 & 64.79 $\pm$ 0.50 \\
% %    Quadruplet + Entropy & \textbf{62.96} $\pm$ 0.58 & \textbf{67.71} $\pm$ 0.25 &  &  \\
%     \midrule 
%     Contrastive \citep{contrastive} & 61.50 $\pm$ 0.17 & 66.45 $\pm$ 0.27 & 75.78 $\pm$ 0.39 & 64.04 $\pm$ 0.13 \\
%     \rowcolor[HTML]{EFEFEF}
%     Contrastive + Entropy & \textbf{63.28} $\pm$ 0.18 & \textbf{67.45} $\pm$ 0.29 & \textbf{76.90} $\pm$ 0.38 & \textbf{65.06} $\pm$ 0.15 \\
%     \midrule
%     Margin (D, $\beta=1.2$) \citep{wu2017sampling} & 63.09 $\pm$ 0.46 & 68.21 $\pm$ 0.33 & 79.86 $\pm$ 0.33 & 67.36 $\pm$ 0.34 \\
%     \rowcolor[HTML]{EFEFEF}
%     Margin (D, $\beta=1.2$) + Entropy & \textbf{64.96} $\pm$ 0.33 & \textbf{69.47} $\pm$ 0.13 & \textbf{82.47} $\pm$ 0.09 & \textbf{68.92} $\pm$ 0.22 \\
%     \midrule
%     Multisimilarity \citep{multisimilarity} & 62.80 $\pm$ 0.70 & 68.55 $\pm$ 0.38 & 81.68 $\pm$ 0.19 & 69.43 $\pm$ 0.38 \\
%     \rowcolor[HTML]{EFEFEF}
%     Multisimilarity + Entropy & \textbf{65.87} $\pm$ 0.45 & \textbf{70.49} $\pm$ 0.16 & \textbf{82.20} $\pm$ 0.15 & \textbf{70.51} $\pm$ 0.25 \\
%     \bottomrule
%     \end{tabular}
%     \label{tab:DML_resutls}
%     \end{minipage}
%  \end{table*}




\begin{table*}[t]
    \caption{\textbf{Literature Comparison}. We show that Entropy-Regularization can provide strong performance boosts on baseline objectives to reach and even improve upon state-of-the-art methods in DML.}
    \setlength\tabcolsep{1pt}
    \footnotesize
    \centering
% \resizebox{\textwidth}{!}{
 \begin{tabular}{l||c|c|c||c|c|c}
     \toprule
     \textbf{Benchmarks} $\rightarrow$ & \multicolumn{3}{c||}{CUB200-2011} & \multicolumn{3}{c}{CARS196}\\
     \midrule
     \textbf{Methods} $\downarrow$ & R@1 & R@2 & NMI & R@1 & R@2 & NMI\\
     \midrule
     \hline
     %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
     \multicolumn{7}{>{\columncolor[gray]{.8}}l}{\textbf{ResNet50-128}} \\
     \hline
     \rowcolor{vvlightgray}
     Div\&Conq \citep{Sanakoyeu_2019_CVPR}  & 65.9 & 76.6 & 69.6 & 84.6 & 90.7 & 70.3\\
     \rowcolor{vvlightgray}
     MIC \citep{roth2019mic}                        & 66.1 & 76.8 & 69.7 & 82.6 & 89.1 & 68.4\\
     \rowcolor{vvlightgray}
     PADS \citep{roth2020pads}              & 67.3 & 78.0 & 69.9 & 83.5 & 89.7 & 68.8\\
     \hline
     Multisimilarity+Entropy                & 66.3 $\pm$ 0.4 & 77.1 $\pm$ 0.4 & 70.5 $\pm$ 0.3 & 84.0 $\pm$ 0.2 & 90.6$\pm$ 0.4 & 71.3$\pm$0.5\\
    %  S2SD-MSIM+Entropy                      & 68.6 $\pm$ 0.3 & 79.0 $\pm$ 0.3 & 72.9 $\pm$ 0.4 & 86.6 $\pm$ 0.3 & 92.3$\pm$ 0.4 & 73.2$\pm$0.4\\
    %  R-Margin+Entropy                       & 66.7 $\pm$ 0.3 & 77.3 $\pm$ 0.3 & 70.5 $\pm$ 0.2 & 84.4 $\pm$ 0.3 & 90.5 $\pm$ 0.3 & 70.9 $\pm$ 0.4\\
     \midrule
     \hline
     %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    %  \multicolumn{7}{>{\columncolor[gray]{.8}}l}{\textbf{ResNet50-512}} \\
    %  \hline
    %  \rowcolor{vvlightgray}
    %  EPSHN \citep{epshn}                     & 64.9 & 75.3 &  -   & 82.7 & 89.3 &  - \\
    %  \rowcolor{vvlightgray}
    %  NormSoft \citep{zhai2018classification} & 61.3 & 73.9 &  -   & 84.2 & 90.4 &  - \\
    %  \rowcolor{vvlightgray}
    %  DiVA \citep{milbich2020diva}            & 69.2 & 79.3 & 71.4 & 87.6 & 92.9 & 72.2 \\
    %  \hline
    %  Multisimilarity+Entropy                & 67.8 $\pm$ 0.4 & 78.1 $\pm$ 0.3 & 71.5 $\pm$ 0.3 & 85.8 $\pm$0.2 & 91.6$\pm$0.3 & 72.5$\pm$0.5\\
    %  S2SD-MSIM+Entropy                      & 69.5 $\pm$ 0.3 & 79.8 $\pm$ 0.4 & 72.6 $\pm$ 0.5 & 88.1 $\pm$0.3 & 92.8$\pm$0.4 & 74.2$\pm$0.4\\
    %  R-Margin+Entropy                       & - & - & - & - & - & -\\
    %  \midrule
    %  \hline
     %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
     \multicolumn{7}{>{\columncolor[gray]{.8}}l}{\textbf{Inception-BN-512}} \\
     \hline
     \rowcolor{vvlightgray}
     Multisimilarity \citep{multisimilarity} & 65.7 & 77.0 & - & 84.1 & 90.4 & - \\     
     \rowcolor{vvlightgray}
     Softtriple \citep{softriple}            & 65.4 & 76.4 & 69.3  & 84.5 & 90.7 & 70.1\\
     \rowcolor{vvlightgray}
     Group \citep{elezi2019group}            & 65.5 & 77.0 & 69.0  & 85.6 & 91.2 & 72.7\\     
     \hline
     Multisimilarity+Entropy                 & 68.5$\pm$0.3 & 79.1$\pm$0.3 & 71.7$\pm$0.5 & 85.8 $\pm$0.3 & 91.6$\pm$0.3 & 72.2$\pm$0.5\\
    %  Multisimilarity+S2SD+Entropy          & 69.4$\pm$0.3 & 80.2$\pm$0.2 & 72.6$\pm$0.3 & 88.0 $\pm$0.3 & 93.2$\pm$0.3 & 74.2$\pm$0.4\\
    %  R-Margin+Entropy                      & 68.6$\pm$0.2 & - & - & - & - & -\\
     \bottomrule
\end{tabular}

\vspace{-10pt}
\label{tab:sota}
\end{table*}

==> tables/dml_table_2.tex <==
\begin{table*}[t!]
 \small
   \setlength\tabcolsep{1.8pt}
   \centering
%   \resizebox{\textwidth}{!}{
    \caption{\textbf{Deep Metric Learning (Zero-Shot Generalization)}. \textbf{1)} Evaluation of max-entropy regularization on strong deep metric learning baseline objectives with a ResNet-50 backbone \citep{resnet} on two standard benchmarks: CUB200-2011 \citep{birds} \& CARS196 \citep{cars}.
    We report mean Recall@1 and Normalized Mutual Information (NMI).
    All baseline scores are taken from \cite{roth2020revisiting}, and 
    their 
    \href{https://github.com/Confusezius/Revisiting_Deep_Metric_Learning_PyTorch}{official released code}
    is used to run all experiments without any fine-tuning. \textbf{2)} We show that max-entropy regularization can provide strong performance boosts on baseline objectives to reach and even improve upon state-of-the-art methods in DML, measured on two standard setups with a ResNet-50 backbone and an Inception-V1 network with frozen Batch-Normalization.}
    
\begin{tabular}{l || c | c || c | c}
 \toprule
 \multirow{2}{*}{\textbf{1) Ablation Study}} & \multicolumn{2}{c||}{CUB200-2011} & \multicolumn{2}{c}{CARS196}\\
 \cmidrule{2-5}
 & R@1 & NMI & R@1 & NMI\\
 \midrule
\rowcolor{vvlightgray} 
Softmax \citep{softmax} & 61.7 $\pm$ 0.3 & 66.8 $\pm$ 0.4 & 78.9 $\pm$ 0.3 & 66.4 $\pm$ 0.3 \\
Softmax + Entropy &  \textbf{65.0} $\pm$ 0.1 & \textbf{68.8} $\pm$ 0.2 & \textbf{80.6} $\pm$ 0.2 & \textbf{68.3} $\pm$ 0.2 \\
%    Quadruplet \citep{qaudrupletloss} & 61.71 $\pm$ 0.63 & 66.60 $\pm$ 0.41 & 76.34 $\pm$ 0.27 & 64.79 $\pm$ 0.50 \\
%    Quadruplet + Entropy & \textbf{62.96} $\pm$ 0.58 & \textbf{67.71} $\pm$ 0.25 &  &  \\
% \midrule 
% Contrastive \citep{contrastive} & 61.5 $\pm$ 0.2 & 66.5 $\pm$ 0.3 & 75.8 $\pm$ 0.4 & 64.0 $\pm$ 0.2 \\
% \rowcolor[HTML]{EFEFEF}
% Contrastive + Entropy & \textbf{63.3} $\pm$ 0.2 & \textbf{67.5} $\pm$ 0.3 & \textbf{76.9} $\pm$ 0.4 & \textbf{65.1} $\pm$ 0.2 \\
\midrule
\rowcolor{vvlightgray}
Margin (D, $1.2$) \citep{wu2017sampling} & 63.1 $\pm$ 0.5 & 68.2 $\pm$ 0.3 & 79.9 $\pm$ 0.3 & 67.4 $\pm$ 0.3 \\
Margin (D, $1.2$) + Entropy & \textbf{65.0} $\pm$ 0.3 & \textbf{69.5} $\pm$ 0.2 & \textbf{82.5} $\pm$ 0.1 & \textbf{68.9} $\pm$ 0.2 \\
\midrule
\rowcolor{vvlightgray}
Multisimilarity \citep{multisimilarity} & 62.8 $\pm$ 0.7 & 68.6 $\pm$ 0.4 & 81.7 $\pm$ 0.2 & 69.4 $\pm$ 0.4 \\
Multisimilarity + Entropy & \textbf{65.4} $\pm$ 0.4 & \textbf{70.3} $\pm$ 0.3 & \textbf{82.2} $\pm$ 0.2 & \textbf{70.5} $\pm$ 0.3 \\
\bottomrule
\toprule
\multirow{2}{*}{\textbf{2) Literature Comparison}} & \multicolumn{2}{c||}{CUB200-2011} & \multicolumn{2}{c}{CARS196}\\
\cmidrule{2-5}
& R@1 & NMI & R@1 & NMI\\
\midrule
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\multicolumn{5}{>{\columncolor[gray]{.8}}l}{\textbf{ResNet50-128}} \\
\hline
\rowcolor{vvlightgray}
Div\&Conq \citep{Sanakoyeu_2019_CVPR}  & 65.9 & 69.6 & \textbf{84.6} & 70.3\\
\rowcolor{vvlightgray}
MIC \citep{roth2019mic}                        & 66.1 & 69.7 & 82.6 & 68.4\\
\rowcolor{vvlightgray}
PADS \citep{roth2020pads}              & \textbf{67.3} & 69.9 & 83.5 & 68.8\\
\hline
Multisimilarity+Entropy                & 66.3 $\pm$ 0.4 & \textbf{70.5} $\pm$ 0.3 & 84.0 $\pm$ 0.2 & \textbf{71.3} $\pm$ 0.5\\
\midrule
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\multicolumn{5}{>{\columncolor[gray]{.8}}l}{\textbf{Inception-BN-512}} \\
\hline
\rowcolor{vvlightgray}
Multisimilarity \citep{multisimilarity} & 65.7 & - & 84.1 & - \\     
\rowcolor{vvlightgray}
Softtriple \citep{softriple}            & 65.4 & 69.3  & 84.5 & 70.1\\
\rowcolor{vvlightgray}
Group \citep{elezi2019group}            & 65.5 & 69.0  & 85.6 & 72.7\\     
\hline
Multisimilarity+Entropy                 & \textbf{68.5} $\pm$ 0.3 & \textbf{71.7} $\pm$ 0.5 & \textbf{85.8} $\pm$ 0.3 & 72.2 $\pm$ 0.5\\
%  Multisimilarity+S2SD+Entropy          & 69.4$\pm$0.3 & 80.2$\pm$0.2 & 72.6$\pm$0.3 & 88.0 $\pm$0.3 & 93.2$\pm$0.3 & 74.2$\pm$0.4\\
\bottomrule
\end{tabular}
\label{tab:DML_results}
\end{table*}

==> tables/dml_table_3.tex <==
\begin{table*}[t!]
 \small
   \setlength\tabcolsep{1.8pt}
   \centering
    \caption{\textbf{Deep Metric Learning (Zero-Shot Generalization)}. \textbf{1)} Evaluation of max-entropy regularization on strong deep metric learning baseline objectives with a ResNet-50 backbone \citep{resnet} on two standard benchmarks: CUB200-2011 \citep{birds} \& CARS196 \citep{cars}.
    We report mean Recall@1 and Normalized Mutual Information (NMI).
    All baseline scores are taken from \cite{roth2020revisiting}, and 
    their 
    \href{https://github.com/Confusezius/Revisiting_Deep_Metric_Learning_PyTorch}{official released code}
    is used to run all experiments without any fine-tuning. \textbf{2)} We show that max-entropy regularization can provide strong performance boosts on baseline objectives to reach and even improve upon state-of-the-art methods in DML.}

\resizebox{0.49\textwidth}{!}{    
\begin{tabular}{l || c | c || c | c}
 \toprule
 \multirow{2}{*}{\textbf{1) Ablation Study}} & \multicolumn{2}{c||}{CUB200-2011} & \multicolumn{2}{c}{CARS196}\\
 \cmidrule{2-5}
 & R@1 & NMI & R@1 & NMI\\
 \midrule
\rowcolor{vvlightgray} 
Softmax \citep{softmax} & 61.7$\pm$0.3 & 66.8$\pm$0.4 & 78.9$\pm$0.3 & 66.4$\pm$0.3 \\
Softmax + Entropy &  \textbf{65.0}$\pm$0.1 & \textbf{68.8}$\pm$0.2 & \textbf{80.6}$\pm$0.2 & \textbf{68.3}$\pm$0.2 \\
%    Quadruplet \citep{qaudrupletloss} & 61.71$\pm$0.63 & 66.60$\pm$0.41 & 76.34$\pm$0.27 & 64.79$\pm$0.50 \\
%    Quadruplet + Entropy & \textbf{62.96}$\pm$0.58 & \textbf{67.71}$\pm$0.25 &  &  \\
\midrule 
Contrastive \citep{contrastive} & 61.5$\pm$0.2 & 66.5$\pm$0.3 & 75.8$\pm$0.4 & 64.0$\pm$0.2 \\
\rowcolor[HTML]{EFEFEF}
Contrastive + Entropy & \textbf{63.3}$\pm$0.2 & \textbf{67.5}$\pm$0.3 & \textbf{76.9}$\pm$0.4 & \textbf{65.1}$\pm$0.2 \\
\midrule
\rowcolor{vvlightgray}
Margin (D, $1.2$) \citep{wu2017sampling} & 63.1$\pm$0.5 & 68.2$\pm$0.3 & 79.9$\pm$0.3 & 67.4$\pm$0.3 \\
Margin (D, $1.2$) + Entropy & \textbf{65.0}$\pm$0.3 & \textbf{69.5}$\pm$0.2 & \textbf{82.5}$\pm$0.1 & \textbf{68.9}$\pm$0.2 \\
\midrule
\rowcolor{vvlightgray}
Multisim. \citep{multisimilarity} & 62.8$\pm$0.7 & 68.6$\pm$0.4 & 81.7$\pm$0.2 & 69.4$\pm$0.4 \\
Multisim. + Entropy & \textbf{65.4}$\pm$0.4 & \textbf{70.3}$\pm$0.3 & \textbf{82.2}$\pm$0.2 & \textbf{70.5}$\pm$0.3 \\
\bottomrule
\end{tabular}}
%%%%%%%%%%%%%%%%%
\hspace{0.1em}
%%%%%%%%%%%%%%%%%
\resizebox{0.49\textwidth}{!}{
\begin{tabular}{l || c | c || c | c}
\toprule
\multirow{2}{*}{\textbf{2) Literature Comparison}} & \multicolumn{2}{c||}{CUB200-2011} & \multicolumn{2}{c}{CARS196}\\
\cmidrule{2-5}
& R@1 & NMI & R@1 & NMI\\
\midrule
\hline
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\multicolumn{5}{>{\columncolor[gray]{.8}}l}{\textbf{ResNet50-128}} \\
\hline
\rowcolor{vvlightgray}
D\&C \citep{Sanakoyeu_2019_CVPR}  & 65.9 & 69.6 & \textbf{84.6} & 70.3\\
\rowcolor{vvlightgray}
MIC \citep{roth2019mic}                & 66.1 & 69.7 & 82.6 & 68.4\\
\rowcolor{vvlightgray}
PADS \citep{roth2020pads}              & \textbf{67.3} & 69.9 & 83.5 & 68.8\\
\hline
Multisim.+Entropy                & 66.3$\pm$0.4 & \textbf{70.5}$\pm$0.3 & 84.0$\pm$0.2 & \textbf{71.3}$\pm$0.5\\
\midrule
\hline
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\multicolumn{5}{>{\columncolor[gray]{.8}}l}{\textbf{Inception-BN-512}} \\
\hline
\rowcolor{vvlightgray}
Multisim. \citep{multisimilarity} & 65.7 & - & 84.1 & - \\     
\rowcolor{vvlightgray}
Softtriple \citep{softriple}            & 65.4 & 69.3  & 84.5 & 70.1\\
\rowcolor{vvlightgray}
Group \citep{elezi2019group}            & 65.5 & 69.0  & 85.6 & 72.7\\     
\hline
Multisim.+Entropy                 & \textbf{68.5}$\pm$0.3 & \textbf{71.7}$\pm$0.5 & \textbf{85.8}$\pm$0.3 & 72.2$\pm$0.5\\
%  Multisimilarity+S2SD+Entropy          & 69.4$\pm$0.3 & 80.2$\pm$0.2 & 72.6$\pm$0.3 & 88.0 $\pm$0.3 & 93.2$\pm$0.3 & 74.2$\pm$0.4\\
\bottomrule
\end{tabular}}
\label{tab:DML_results}
\end{table*}

==> tables/metadataset_table.tex <==
\begin{table*}[t!]
\setlength\tabcolsep{1.4pt}
\begin{minipage}[c]{\textwidth}
\small
\caption{\textbf{Out-of Distribution Generalization}. Comparison of several network architectures on their performance on OOD Generalization. We report mean accuracy and standard deviation over 5 random seeds. To generate OOD samples, we perform random translations, rotations, and scaling over each test image.}
\centering
   \begin{tabular}{ c | c || c | c || c | c}
     \toprule
    \textbf{ ResNet-18} & + Entropy & \textbf{WideResNet-50} & + Entropy & \textbf{ResNeXt-50} & + Entropy \\
    \midrule
    35.6 $\pm$ 1.2 & \textbf{41.3} $\pm$ 1.3 & 39.6 $\pm$ 1.2 & \textbf{43.9} $\pm$ 0.9 & 40.1 $\pm$ 0.8 & \textbf{43.8} $\pm$ 1.1 \\
    \bottomrule
    \end{tabular}
    \label{tab:ood_results}
\end{minipage}
\end{table*}
